Accelerated Emergence of Evolved Galaxies in Early Overdensities at $z\sim5.7$

We report the identification of two galaxy overdensities at $z\sim5.7$ in the sightline of the galaxy cluster Abell 2744. These overdensities consist of 25 and 17 member galaxies, spectroscopically confirmed with JWST NIRSpec/MSA and NIRCam/WFSS. Each overdensity has a total stellar mass of $\sim2\times10^{10} M_\odot$ and a star formation rate of $\sim200 M_\odot$/yr within a central region of radius $R=2$ Mpc (physical). The sensitive PRISM spectra allow us to identify six galaxies that show weak Ha+[NII] emissions within the overdensities ($27\pm6\%$), whereas the fraction of such galaxies is found significantly lower ($6\pm2\%$) in field samples of the equivalent redshift range. These weak emission line galaxies, dubbed as wELGs, exhibit a strong continuum break at $4000$AA rest-frame, a characteristic feature of evolved stellar populations. The high observed fraction of wELGs in the two overdensities is consistent with the idea that high-density environments are an ideal site where galaxies can accelerate their evolutionary pace compared to field analogs. Our study pinpoints an early onset of environmental effects, already important within one billion years after the Big Bang, and provides a complementary perspective on the emergence of quenched, massive galaxies at lower redshifts. Potential contributions from black hole accretion feedback to the reduction of star formation activity are discussed, but the connection to the local environments remains unclear.

==> table_linefluxes.tex <==
\begin{deluxetable*}{ccccc}
\tabletypesize{\footnotesize}
\tablewidth{-2pt}
\tablecaption{
Emission line measurements of \id.
}
\tablehead{
\colhead{Line} & \colhead{IP} & \colhead{Flux} & \colhead{$\sigma$} & \colhead{EW$_0$}\\
\colhead{} & \colhead{eV} & \colhead{$10^{-19}$\,erg/s/cm$^2$} & \colhead{km/s} & \colhead{$\mathrm{\AA}$}
}
\startdata
${\rm HeII}_{4686}$ & 54.4 & $17.4 \pm 5.0$ & $1020.4 \pm 128.3$ & $37.8 \pm 6.0$\\
${\rm [ArIV]}_{4711}$ & 40.74 & $<2.6$ & -- & --\\
${\rm HeI}_{4714}$ & 24.6 & $4.8 \pm 2.8$ & $317.0 \pm 27.6$ & $2.4 \pm 1.6$\\
${\rm [ArIV]}_{4740}$ & 40.74 & $4.3 \pm 2.8$ & $312.2 \pm 40.0$ & $2.3 \pm 1.5$\\
${\rm H\beta}_{4861}$ & 3.4 & $174.5 \pm 3.7$ & $159.7 \pm 1.3$ & $130.3 \pm 1.0$\\
${\rm HeI}_{4922}$ & 24.6 & $<2.1$ & -- & --\\
${\rm [OIII]}_{4959+5007}$ & 35.1 & $1271.1 \pm 19.6$ & $144.7 \pm 0.4$ & $228.0 \pm 0.7$\\
${\rm [OI]}_{5577}$ & 0 & $<1.5$ & -- & --\\
${\rm [NII]}_{5755}$ & 14.5 & $1.0 \pm 0.8$ & $91.1 \pm 21.4$ & $1.1 \pm 0.3$\\
${\rm HeI}_{5876}$ & 24.6 & $21.3 \pm 1.4$ & $142.9 \pm 4.4$ & $23.8 \pm 0.7$\\
${\rm [OI]}_{6300}$ & 0 & $10.1 \pm 0.6$ & $151.9 \pm 6.5$ & $14.0 \pm 0.5$\\
${\rm [SIII]}_{6312}$ & 19.1 & $3.0 \pm 0.8$ & $154.8 \pm 27.6$ & $4.1 \pm 0.6$\\
${\rm [OI]}_{6364}$ & 0 & $2.9 \pm 0.2$ & $151.9 \pm 6.5$ & $4.0 \pm 0.1$\\
${\rm SiII}_{6373}$ & 8.2 & $1.4 \pm 0.8$ & $204.0 \pm 42.5$ & $2.1 \pm 0.6$\\
${\rm [NII]}_{6548+6583}$ & 14.5 & $52.5 \pm 5.3$ & $150.7 \pm 2.2$ & $29.3 \pm 0.4$\\
${\rm H\alpha}_{6563}$ & 3.4 & $499.1 \pm 7.1$ & $142.7 \pm 0.4$ & $750.2 \pm 2.3$\\
${\rm HeI}_{6678}$ & 24.6 & $5.3 \pm 0.7$ & $128.8 \pm 11.2$ & $7.5 \pm 0.5$\\
${\rm [SII]}_{6716}$ & 10.4 & $24.9 \pm 0.8$ & $137.0 \pm 2.8$ & $36.0 \pm 0.7$\\
${\rm [SII]}_{6731}$ & 10.4 & $22.2 \pm 0.8$ & $133.7 \pm 3.0$ & $32.4 \pm 0.6$\\
${\rm OI}_{7002}$ & 0 & $<0.9$ & -- & --\\
${\rm HeI}_{7065}$ & 24.6 & $8.3 \pm 0.8$ & $126.5 \pm 6.6$ & $14.5 \pm 0.7$\\
${\rm [ArIII]}_{7136}$ & 27.6 & $12.2 \pm 1.0$ & $136.9 \pm 5.2$ & $22.5 \pm 0.8$\\
${\rm HeI}_{7281}$ & 24.6 & $1.5 \pm 0.9$ & $172.3 \pm 36.0$ & $2.8 \pm 0.8$\\
${\rm [OII]}_{7320}$ & 13.6 & $4.9 \pm 0.8$ & $111.2 \pm 12.6$ & $9.5 \pm 0.9$\\
${\rm [OII]}_{7331}$ & 13.6 & $5.0 \pm 0.9$ & $149.6 \pm 18.9$ & $9.4 \pm 1.1$\\
${\rm [NiII]}_{7378}$ & 7.6 & $<0.8$ & -- & --\\
${\rm [NiII]}_{7411}$ & 7.6 & $<0.9$ & -- & --\\
${\rm [ArIII]}_{7751}$ & 27.6 & $1.7 \pm 0.9$ & $91.9 \pm 20.4$ & $3.9 \pm 0.7$\\
${\rm OI}_{7774}$ & 0 & $<1.0$ & -- & --\\
${\rm HeI}_{7816}$ & 24.6 & $<1.1$ & -- & --\\
${\rm HeII}_{8237}$ & 54.4 & $<0.6$ & -- & --\\
${\rm [SIII]}_{9069}$ & 19.1 & -- & -- & --\\
${\rm Pa9}_{9229}$ & 1.5 & $3.8 \pm 0.9$ & $175.9 \pm 19.0$ & $12.5 \pm 1.0$\\
${\rm [SIII]}_{9531}$ & 19.1 & $55.9 \pm 1.5$ & $158.0 \pm 1.5$ & $203.5 \pm 1.7$\\
${\rm Pa\delta}_{10049}$ & 1.5 & $8.1 \pm 0.6$ & $127.7 \pm 4.5$ & $29.7 \pm 1.0$\\
${\rm HeI}_{10830}$ & 24.6 & $66.3 \pm 1.1$ & $155.6 \pm 1.1$ & $263.6 \pm 1.8$\\
${\rm Pa\gamma}_{10938}$ & 1.5 & $14.0 \pm 0.6$ & $123.7 \pm 2.5$ & $60.0 \pm 1.1$\\
${\rm OI}_{11287}$ & 0 & $1.0 \pm 0.5$ & $162.7 \pm 18.0$ & $5.0 \pm 1.2$\\
${\rm [FeII]}_{12567}$ & 7.9 & $3.3 \pm 0.4$ & $142.9 \pm 11.9$ & $18.0 \pm 1.7$\\
${\rm HeI}_{12790}$ & 24.6 & $1.9 \pm 0.8$ & $133.6 \pm 16.2$ & $8.8 \pm 1.3$\\
${\rm Pa\beta}_{12818}$ & 1.5 & $29.2 \pm 1.0$ & $121.1 \pm 1.8$ & $135.4 \pm 1.8$\\
\enddata
\tablecomments{
% Fluxes are in units of $10^{-19}$\,erg/s/cm$^2$. 
Flux errors are $2\,\sigma$. 
The reported fluxes are not corrected for magnification. Attenuation has been corrected using $A_V=0.43$. EW$_0$: Rest-frame equivalent width.
}\label{tab:lines}
\end{deluxetable*}

==> table_phys.tex <==
\begin{deluxetable*}{ccc}
\tabletypesize{\footnotesize}
\tablecolumns{3}
\tablewidth{0pt}
\tablecaption{
Physical properties of \id}
\tablehead{
\colhead{Property} & \colhead{Unit} & \colhead{Measurement}\\
\colhead{} & \colhead{} & \colhead{}
}
\startdata
\cutinhead{Host properties}
R.A. & degree & $1.773851e+02$\\
Dec. & degree & $2.237533e+01$\\
$M_*$ & $\log M_\odot$ & $9.6_{-0.1}^{+0.2}$\\
$A_{V, \mathrm{SED}}$ & mag & $0.3_{-0.1}^{+0.1}$\\
$\beta_{\mathrm{UV}}$ &  & $-1.7_{-0.1}^{+0.1}$\\
$R_e$ & kpc & $0.7_{-0.1}^{+0.1}$\\
\cutinhead{ISM properties}
$A_{V,\mathrm{HII, SMC}}$ & mag & $0.4$\\
$A_{V,\mathrm{HII, LMC}}$ & mag & $0.6$\\
$n_{e}(\mathrm{[SII]})$ & $10^{2}$cm$^{-3}$ & $2.48_{-0.22}^{+0.20}$\\
$T_{e}(\mathrm{[SIII]})$ & $10^{4}$\,K & $1.47_{-0.11}^{+0.13}$\\
$T_{e}(\mathrm{[NII]})$ & $10^{4}$\,K & $1.38_{-0.25}^{+0.39}$\\
$T_{e}(\mathrm{[OIII]})_\mathrm{[NII]}$ & $10^{4}$\,K & $1.48_{-0.33}^{+0.44}$\\
$T_{e}(\mathrm{[OIII]})_\mathrm{[SIII]}$ & $10^{4}$\,K & $1.50_{-0.10}^{+0.14}$\\
$T_{e}(\mathrm{[OI]})$ & $10^{4}$\,K & $<1.99$\\
$12 + \mathrm{\log (O^+/H^+)}$ &  & $7.34_{-0.04}^{+0.04}$\\
$12 + \mathrm{\log (O^{2+}/H^+)}$ &  & $7.78_{-0.10}^{+0.08}$\\
$12 + \mathrm{\log (O/H)}$ &  & $7.92_{-0.08}^{+0.07}$\\
$\mathrm{\log (S^+/H^+)}$ &  & $5.49_{-0.01}^{+0.01}$\\
$\mathrm{\log (S^{2+}/H^+)}$ &  & $5.98_{-0.05}^{+0.05}$\\
$\mathrm{\log (S/O)}$ &  & $-1.76_{-0.04}^{+0.04}$\\
$\mathrm{\log (N^+/H^+)}$ &  & $6.31_{-0.23}^{+0.22}$\\
$\mathrm{\log (N/O)_\mathrm{[SIII]}}$ &  & $-1.09_{-0.09}^{+0.09}$\\
$\mathrm{\log (N/O)_\mathrm{[NII]}}$ &  & $-1.04_{-0.23}^{+0.22}$\\
$\mathrm{\log (Ar^{2+}/H^+)}$ &  & $5.47_{-0.02}^{+0.02}$\\
$\mathrm{\log (Ar/O)}$ &  & $-2.40_{-0.02}^{+0.02}$\\
$n(\mathrm{H^+})/n(\mathrm{H^0})$ &  & $248$\\
\cutinhead{ISM properties (He~I)}
$T_{e}(\mathrm{HeI,6678})$ & $10^{4}$\,K & $2.01_{-0.82}^{+0.98}$\\
$T_{e}(\mathrm{HeI,5876})$ & $10^{4}$\,K & $1.74_{-0.78}^{+1.25}$\\
$\tau_{3889}$ &  & $2.80_{-0.70}^{+0.80}$\\
$A_{V, \mathrm{HeI, SMC}}$ & mag & $0.5$\\
\cutinhead{Starformation rates}
$\mathrm{SFR_{SED}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.56_{-0.03}^{+0.03}$\\
$\mathrm{SFR_{Hb4861}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.29 \pm {0.01}$\\
$\mathrm{SFR_{Ha6563}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.29 \pm {0.01}$\\
$\mathrm{SFR_{Pa99229}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.36 \pm {0.41}$\\
$\mathrm{SFR_{Pad10049}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.39 \pm {0.06}$\\
$\mathrm{SFR_{Pag10938}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.24 \pm {0.02}$\\
$\mathrm{SFR_{Pab12818}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.30 \pm {0.01}$\\
$\mathrm{SFR_{HeI5876}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.36 \pm {0.02}$\\
$\mathrm{SFR_{HeI6678}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.33 \pm {0.14}$\\
$\mathrm{SFR_{HeI7065}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.36 \pm {0.11}$\\
$\mathrm{SFR_{HeI7281}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.32 \pm {2.47}$\\
$\mathrm{SFR_{HeI10830}}$ & $\log M_\odot {\rm yr^{-1}}$ & $1.32 \pm {0.01}$\\
\enddata
\tablecomments{
Measurements are corrected for magnification using $\mu=1.34$ (Sec.~\ref{sec:data})
}\label{tab:phys}
\end{deluxetable*}
